Remote Learners, Home Makers: How Digital Fabrication Was Taught Online During a Pandemic

Digital fabrication courses that relied on physical makerspaces were severely disrupted by COVID-19. As universities shut down in Spring 2020, instructors developed new models for digital fabrication at a distance. Through interviews with faculty and students and examination of course materials, we recount the experiences of eight remote digital fabrication courses. We found that learning with hobbyist equipment and online social networks could emulate using industrial equipment in shared workshops. Furthermore, at-home digital fabrication offered unique learning opportunities including more iteration, machine tuning, and maintenance. These opportunities depended on new forms of labor and varied based on student living situations. Our findings have implications for remote and in-person digital fabrication instruction. They indicate how access to tools was important, but not as critical as providing opportunities for iteration; they show how remote fabrication exacerbated student inequities; and they suggest strategies for evaluating trade-offs in remote fabrication models with respect to learning objectives.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> sections/findings.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=0.85\textwidth]{figures/CHI2021_fullpageFigure-lowres.png}
  %\caption{A) Yanrong Chen’s sculpture of interlocking chains and birdcages in \hcde B) Design of a space frame from a single node to the robotic assembly in \raw C) \sam's bioplastic from 3D printed molds in \mat D) \skylar, Shiley Einav, Julian Ochoa and Ellie Prince's marble maze CAD project in \me E) Pippa Kelmenson making conductive silicone using a fork in a drill and a take-out container in \tangible F) Aidan Lincoln's vinyl lamp in \itp G) Samuel Rushenberg's pen holder designs for KUKA robotic arm in \arch H) Jaideep Cherukuri, Scout Handford, Jahangir Abbas Mohammed, Abrar Syed \& Miyuki Weldon Amazing Cane project to enhance white canes in \desinv I) Kat Sung's cyberpunk mask from recycled objects in \desma }
  \caption{A wide range of student work was produced in remote digital fabrication classes in Spring 2020. A) A sculpture with many interlocking parts iteratively printed in \hcde B) Design of a space frame from a single node to robotic assembly in \raw C) \sam's bioplastic cast in 3D printed molds in \mat D) A marble maze collaborative CAD project in \me E) Conductive silicone mixed with a fork-drill with kitchen containers in \tangible F) Vinyl lamp iterations in \itp G) Pen holder designs for a robotic arm in \arch H) Combining electronics and 3D prints in \desinv I) Using found and recycled objects in \desma.} % I removed non-macro names for now too
  \label{fig:figure1}
\end{figure*}

\section{Remote Instruction with At-Home 3D Printers}
\input{sections/internalfindings}

\section{Remote Instruction with Other Fabrication Models}%External Models of Remote Fabrication Instruction}
%~\jj{better title needed}
\input{sections/externalfindings}













==> sections/findings_sections/curriculumchanges.tex <==
~\jj{remove- move to other sections?}
Instructors had to adapt their course curriculum to a remote learning environment, which they sometimes were able to plan slightly ahead of time (as was the case for ME102, R.A.W. and xx) and sometimes in the midst of the semester (Architectural Robotics, DESINV and xx). Regardless of their course timeline, all instructors had to shift their teaching approaches and experiment with new fabrication workflows. Most instructors also faced challenges when planning their course in the midst of a global pandemic.

Instructors who opted for on-demand fabrication services, such as Vivek Rao, Adam Hutz and George Moore for DESINV 190/290 at Berkeley and Mark Cutkosky for ME102 at Stanford, reported changes in their course's fabrication workflow. In Mark's class, one assignment required to send the students' designs to a 3D fabrication center and then to send the printed parts back to students in the US and in other countries. This approach worked well but also meant additional labor for the instructor and the teaching assistants, who had to collect and sometimes debug the student's designs, and caused a two weeks delay in the course timeline. For Vivek's, Adam's and George's class, cost and turnaround time were important factors when choosing the right fabrication service, as there were many additional steps involved to get parts into the hands of the students: "[W]e needed students to be able to submit their files to us. We needed to upload those files. Those files needed to be processed by a manufacturer and then shipped" reports Adam. Other new workflows involved instructors 

 Shifts in teaching practices included using video to support content delivery, a heavier focus on CAD and/or simulation, extended discussions (as opposed to demos or lectures), and the creation of small groups to provided more targeted assistance. 

Mark from ME102 and his TAs prepared videos to present content to the students at the beginning of each coaching session, which were small group sessions of 6-8 students and a TA. During the sessions, the students watched the video with the TA, who would periodically pause the video to address students' questions, add or clarify content. For Skylar, a student in the class, this format felt more "natural than a normal lecture. To me, I felt I could ask questions and I could participate." Skylar also indicated the class had a heavier emphasis on CAD, something he felt his peers had a higher demand for (rather than prototyping skills) "because that is something that internships ask for."

Simulations were used by some instructors, with limited outcomes. James Coleman, instructor of the Robotic Architecture Workshop at Princeton, used robotics simulation to convey some of the experience of working with large scale industrial machines. But despite leading successful software simulation with the students, James highlighted the practical learning experience that takes place when working with machines: 

\begin{quote}
"Then you send [the code] to the machine and it tries to do it upside down or backwards, or it tries to go through the floor. And all of a sudden you realize that there was a negative value of one of your vectors, you know, could have caused all sorts of damage. So those are the things that, it, it seemed very easy for [the students], right? Like, Oh, well I simulated the robot. I'm like, well, yeah, but does that actually mean that the information, the robot perceived would translate it in the same way?"
\end{quote}

Mark also discussed the limitations of simulation, indicated that "you can in CAD estimate the effect of tolerance stack up, but in fact, there wasn't that much we could do besides sort of consciousness raising about it." Lauren, Shelby's student, who taught Architectural Robotics at Iowa State University, reported that losing access to the campus' fabrication space made her and her classmates rely more heavily on the instructor's feedback to iterate on their designs. Discussion became an important mean of conveying fabrication experience in other classes as well. Skylar describes:

\begin{quote}
"Talking to Mark and the TAs, they really took us through like, “Okay, if you were about to print this, you'd walk over to the printer, you'd stick your USB, you know, you do whatever.” And so I, I did get a feel for that."
\end{quote}

The remote contact with the students drove some instructors to work with smaller groups at a time or to schedule individual check-ins. As discussed above, Mark and his TAs scheduled coaching sessions that focused on 6-8 students. Paul Esposito, instructor of DESMA160 at UCLA, scheduled one-on-one meetings with his students throughout the course, "to make sure that they were doing well or just getting on in terms of the coursework. Any challenges that they had." This individual or more targeted attention often lead to increased participation and a sense of support for students (see Learning opportunities). The emotionally and physically challenging times in which these classes took place often meant that instructors were more accommodating with their students and often modified their expectations of the course outcomes.  "In some ways" says Paul Esposito, "that class was maybe asking like a little bit too much of the students, especially in this very frustrating, stressful time."
 
Instructors faced logistical and resource challenges when transitioning to these teaching approaches. Implementing new workflows and developing ad hoc teaching strategies often meant more labor for the teaching staff. In Mark’s class, using an on-demand fabrication service meant TAs had to test the parts when they came back from the fabrication center and also that they spent more time providing support to their group of students. "The TAs were spending at least an extra sort of half hour per week doing this, [the] tutored video instruction, beyond what they would normally spend, just coaching students and working with them" said Mark. Similarly, the teaching staff for DESINV 190/290 at Berkeley had to run a quality check on the students’ designs before sending them to a vendor. Researching the right fabrication service also meant extra labor for the instructor and TAs Paul Esposito, who fabricated parts for his students with at-home equipment, indicated that this approach might not be a viable solution for future classes: " I think it would become an issue of my hours being overused." Preparing for remote instruction in the Fall of 2020 also means "more work upfront", says Mark Cutkosky, who plans to add 3D printed parts with different infill ratios to the students' making kits to support learning about materials and stiffness. 
    
Institutional and social realities sometimes interfered with the instructors' efforts to plan their class. Shelby Doyle points out:

\begin{quote}
"I think if we were teaching online on purpose rather than kind of as an emergency, I could be really, I could feel more creative about it, you know? Like it would be like fun. Whereas right now I think it's just all wrapped up in so much other, you know, administrative bureaucracy and like societal and it's hard." 
\end{quote}

Acknowledging the current pandemic and taking the appropriate measures to address the new reality of remote instruction is crucial to the effort of planning and teaching high-quality fabrication courses online. 
    
  

==> sections/findings_sections/fabaccess.tex <==
Most of the surveyed courses were originally designed~\jj{which ones weren't? Can we say a number? e.g. 5 of 6?} around digital fabrication resources in a makerspace. In the rapid onset of the pandemic, instructors had to devise alternative means of access to elements resources with minimal planning time and constrained resources. 

%\me and \desma were both planned in relation to other digital fabrication courses from their respective departments. \me is part of a series of three courses designed to teach students the fundamentals of making objects~\jj{is this necessary context? cut?}. 
The short time frame and limited precedent for remote fabrication led 3 instructors to dramatically alter their curriculum and assignments so they could function without digital fabrication access, while retaining  elements of hands on making or digital fabrication. \me's primary focus shifted to collaborative CAD however the instructor and TA still walked students through basic steps required for digital fabrication or provided remote demonstrations.%:``if you were about to print this, you'd walk over to the printer, you'd stick in your USB''~\jj{can we cut this quote?. it's not so compelling and the point is made without it.. 
\paul created an entirely new course (\desma) because his department decided infeasible to to teach the original digital fabrication course in a remote format with limited preparation time. \paul was able to take advantage of the freedom of creating a new course to experiment with remote versions of fabrication that including shipping sewing kits, and printing student designs via his home 3D printers. %Nevertheless, "[he] was allowed to like kind of make up my own selected topics course that was somehow like \textit{Form} affiliated."
\sbt{making it clearer the impacts of this point?}~\jj{i revised. confirm it matches data?}

Instructors efforts to provide students with access to fabrication tools and materials in remote courses were constrained by how their departments managed material sourcing. Pre-pandemic, students in art departments were expected to pay for their own materials. As an instructor in an art school, Ben Light maintained that "we're very upfront, like projects, cost money, you need stuff to make stuff. And and you can work cheap, but you know, you, you, you need to work with something. And we, you know, I'm constantly giving material away that I have built up over the years, but it's not like I can supply a whole class with it either." However, Ben always provides a thorough list of online and local resources for sourcing to students. \sbt{add ways for sourcing in engineering-oriented field?}~\jj{how did this impact what he/ students could do remotely?}

\sbt{need some continuity with previous points} Maker spaces normally provide access to, both, the machines and the expert support for students to learn digital fabrication. Mark mentioned that, for the in-person format of ME102, students “[could] just wander in” the student shops, where “one of the TA’s [would] be holding open shop hours.” 

The loss of access to theses maker spaces generated different reactions from students. When Lauren, one student in the \textit{Arch 438X} course, described an assignment about designing a stable pen holder add-on for a KUKA robotic arm, she mentioned that “without being able to test it on the machine, it just kind of didn't make sense to use that function.” She didn't see the value or the use of developing artifacts that could not be applied to physical equipment and felt, therefore, demotivated to put energy into it. Skylar, a student in ME102, expressed the anxiety associated with sourcing parts and materials from outside his house as he didn't feel inclined “to go to a hardware store and get all of this stuff and leave during quarantine or whatever lockdown to go do all this”. Nevertheless, Shelby saw this limited sourcing context as a creative opportunity to have students re-envisioning forms of production or outcomes with at-home materials.


Different strategies and logistics were then implemented by instructors. In part due to prior expectations of some students, instructors felt the desire to retain some form of machine access or physical outcomes. Discussing the reasons why they decided to keep a tangible component as part of the DESINV 190/290-9 course, Vivek mentioned:


\begin{quote}
    “So there was a real hunger for some kind of, um, you know, some kind of strong finish. And we, you know, looked around and noticed that a lot of classes were doing making decisions similar to what you said and that like, let's step back, let's transition. And I think we made a conscious decision to kind of hold, you know, hold a certain level of, of, you know, expectation and outcomes that we wanted to push for. And I think that, you know, I know that some students like may not have been thrilled with that and then others really excited about, but that was the decision that we made. We really wanted to do our best to preserve some of the original intent because we saw there was a lot of desire from students to meet that.” (Vivek)
\end{quote}

To maintain physical making in the curriculum, a first strategy was to have students or TAs act as technicians for others. In the case of the R.A.W., one student and the two TAs became fabricators on the vinyl cutter for the other 5 participants. However, because the duration of the workshop was short, the fabricators were not able to mail the parts in time “ [s]so they, they photographed the parts and pieces of her cut, did the assembly and then sent back, you know, photographs of the freight”. Mark who also thought about asking TAs to fabricate parts for students was actually concerned about turning them into a fabrication service:

\begin{quote}
    “I need to be a little careful that TAs didn't sign up to become a service, a parenting service. They signed up to become teaching assistants and that's what they want to do. They want to teach and coach nonetheless, I think if we can do at least some fabrication on campus to get stuff sent out to people, I think, I think we should do it.” (Mark)
\end{quote}

In the \textit{ITP-Subtraction} course, some students took the initiative to put in place their own job shop: “one person bought another mill or a Bantam mill and someone bought 3D printer. I don't remember what it was, but they all sort of like, I've got this. If you need a part, I'll run one.”(Ben) But according to Ben, “that ended up not happening as much as I thought it would. I thought that those people would be very popular and again, they, they may one or two things maybe for someone else, but it was mostly, I think everyone just embraced the constraints and lived there.” 

Mentioning he had two 3D printers at home, Paul Esposito was also “hoping that I would be able to kind of fabricate these projects for the students and get in a little bit deeper with some of the projects” but only “two out of 21 [students] that were like really interested in developing their 3D modeling skills.” The minority of students who ended up taking advantage of Paul’s fabrication setup were the ones with already some CAD/FAB expertise. These students were not able to receive the physical parts though. Paul was planning on leaving the parts at UCLA at the end of the quarter if the COVID-19 situation would get better which did not happen.

A second strategy that took place in one the the surveyed course was to use university maker spaces as a job shops for students to order parts. Students in the \textit{Arch 438X} course were able to order 3D printed or laser cut parts from the CCL at Iowa State University. One student pointed out though that this option was only available for pick up directly at the school which made it “really only an option for like a few people”, adding that “a lot of people that I know moved home, which could be, you know, a couple hours away, um, a couple of States away”. According to this student, it was not clear “how many people actually ended up utilizing that” service. 

A third investigated strategy was to send hobbyist machines to students. In the case of the R.A.W., the vinyl cutter sent to three people aimed to approximate elements of industry-grade machines. Discussing the relevance of using the vinyl cutter for students interested in space frames, James said that they “were going to basically use paper as a stand in for sheet metal because it was sort of a strength to weight ratio is pretty similar and even formability is quite similar between paper and sheet metal.”

Mark who didn't end up sending 3D printers to his students viewed the 3D printer “kit itself has opportunities for learning about how you assemble things so that the tolerances are actually achieved and alignment and well, lots of issues it can bring up and heating and heat transfer”.

The at-home fabrication strategy showed evidences that students who received machines were able to use them at greater rates, and at irregular hours. Indeed, Ben believed that living with the machine had learning opportunities: 

\begin{quote}
    “The thing I loved about the vinyl cutters more than anything that actually came out of it is that students got to live with the machines. And I think that's really the only way to, to, to get good at it. Right? Like you get a crazy idea and then you immediately make it. And you're like, no, you stay up till four in the morning and you keep working on it. I mean, you somehow learn it inside and out. It starts having quirks that, you know, and that's something that never happened in the past because no one had the machines, they did it here and then they left and there were 10 people behind them waiting for their turn. So access, they had an, you know, parallel access to their machines. And that was huge. I think it just may not have been the machine they wanted, but having total access to something and the time to you know, being trapped in doors with nothing but your vinyl cutter, you know, that learned it.”
\end{quote}

However, the presence of machines at home could also be disruptive to home life for instructors and students. Shelby mentioned zoom calls getting noisy because of the 3D printers running near her, which she could still hear at night when going to bed.

\sbt{living situation here??}

James also mentioned that hobbyist machines, specifically the vinyl cutter, could be overly constraining for university level courses and workshops. Mentioning the automatic scaling done by the machine on larger files, James suggested that the machine "was making a lot of assumptions about us as users, and that were extremely annoying because it wasn't an open software." So, with the participants, they ended up "figuring out the smoothest workflow through and nesting to this size of sheet, even though we could cut it actually cut larger."

A fourth employed strategies involved shipping tools, materials and digitally fabricated parts but the ordering and shipping were often done on the fly with little time for planning ahead. Mark shipped “a marble to everybody” for one assignment and, for another CAD exercise, the instruction team “took all the students' designs, collected them, sent them out to an online 3d fabrication center, 3d hubs, and, uh, and then sent the parts out to the students”. Mark also mailed some testing kits, including a dial gauge and clamps, to each TA "so that they live with their little group could do the test on each crank" designed by their respective students.

%"That was the best we could do in other words, for their six to eight students. So we did send out a, a, a test kit, a dial gauge and, uh, and clamps and so on for each of the TAs, so that they live with their little group could do the test on each crank, but there was just no way we could do, but to each student, we just, we just didn't have time for this last spring." \sbt{add this somehow}

The DESINV 190/290-9 course also parts from an online fabrication vendor to the students. \sbt{add stuff}

Depending on online fabrication services caused some delay to happen, which affected the potential for students to iterate on their design. Mark mentioned that "[t]he students got their parts, but they finally got them almost two weeks later that I was hoping they would". One of his students confirmed that "because of the quarter system, things just move so fast that you weren't expecting, like ordering something on some sort of printing service and have it shipped to every student. It's like, Oh, well there went to half of the quarter." Adam at Berkeley added that these delays would constrain students to "only one iteration on the timeline". \sbt{maybe explain why iteration is important?}

Paul also sent sewing kits to students who didn't have some already. \sbt{add stuff}

Finally, some courses expected students to have basics tools and materials at home. Mark mentioned: "We, we, we mandated that every student in the class should have a very low tech kit, uh, an Exacto knife, hot note, glue guns, some cardboard, masking tape ruler." However, one student in the ME102 course noted that home is not necessarily the best space for prototyping: "I'm not gonna cut a piece of cardboard on my mom's wood dining table. Like it's not, you know, it doesn't really make sense. There's not really a lot of places in my house where I can do that kind of work. I'm not going to buy a drill press."







%How people got their equipment. What was the experience of living with it.
%Pre-pandemic models of access to fabrication equipment.
%\begin{itemize}
  %  \item Courses  built up around the existence of a maker-space or fabrication resources
    %Esposito.
    %Skylar in explaining the ME course. 
   
 %   \item Makerspace provided access both to machines and to support and expertise.
    %https://docs.google.com/document/d/1OIt0d5Ve4bGTJas2ZIwHXHp7bJlf-1sTJojdwwCfF1I/edit?disco=AAAAKIXEMnQ
    
 %   \item Differences in how materials are managed. Art students are responsible for paying for their own materials, but instructor provides support for sourcing.
    %https://docs.google.com/document/d/1svv9sfaZ8NtMqLYOEsXdhRuiJxVOhKP2_ZdHqkM_DYM/edit?disco=AAAAKLx5Nvk
    %https://docs.google.com/document/d/1svv9sfaZ8NtMqLYOEsXdhRuiJxVOhKP2_ZdHqkM_DYM/edit?disco=AAAAKLx5Nvk
    
%\end{itemize}

%Reactions to losing access to makerspaces
%\begin{itemize}
 %   \item Reduced motivation to develop artifacts that could not be applied to physical equipment, and increased difficulty in design process.
    %https://docs.google.com/document/d/1pi8dNLhy76DvkQUTEmOegwmyoTJq7epPQACGot_1bm8/edit?disco=AAAAG3pc_SQ
    %https://docs.google.com/document/d/1pi8dNLhy76DvkQUTEmOegwmyoTJq7epPQACGot_1bm8/edit?disco=AAAAG3pc_SU
    
    %\item shift to re-envisioning forms of production or outcomes with at home materials.
    %https://docs.google.com/document/d/1dJM5lyaog2zqkmpr-qCYtxUG2W1mm2wX1pICl1HFrXw/edit?disco=AAAAG3694gg
    
    %\item Anxiety / uncertainty of going to store to source parts and materials.
    %https://docs.google.com/document/d/1EysxU4c-bFz1sgeEMxlNtHQM9mYWu1eXF8402NgCakI/edit?disco=AAAAKLMjsmY
%\end{itemize}


%Strategies and logistics for getting students access to equipment.
%\begin{itemize}
    
     %\item Instructor desire to retain machine access in some form, in part due to prior expectations of some students.
     %https://docs.google.com/document/d/1svv9sfaZ8NtMqLYOEsXdhRuiJxVOhKP2_ZdHqkM_DYM/edit?disco=AAAAKLx5NvY this is wor Fall quarter though... not sure we should use it in this context.
     %Berkeley
     
    %\item Makerspace becoming jobshop and students or TAs becoming technicians.
    %https://docs.google.com/document/d/1svv9sfaZ8NtMqLYOEsXdhRuiJxVOhKP2_ZdHqkM_DYM/edit?disco=AAAAKLx4U7w
    %https://docs.google.com/document/d/1bFfPoLLz9gunDBTSW4dAXXWyQPQ3uSr-pSXxcVWAhEs/edit?disco=AAAAG367t40
    
    %\item providing some students with access to hobbyist machines that approximated elements of industry grade machines.
    %https://docs.google.com/document/d/1svv9sfaZ8NtMqLYOEsXdhRuiJxVOhKP2_ZdHqkM_DYM/edit?disco=AAAAG5UKT7M
    
    %\item Shipping students tools (sewing kits), materials (marbles), digitally fabricated parts (final projects for Berkeley class though shipping was often done on the fly with little time for planning.
    %https://docs.google.com/spreadsheets/d/1Gp0rCxjDpsg8qkZbCT3GBPLVROr9slUIcWHlF9cNC8Y/edit?disco=AAAAKIXEMmY
    %https://docs.google.com/spreadsheets/d/1Gp0rCxjDpsg8qkZbCT3GBPLVROr9slUIcWHlF9cNC8Y/edit?disco=AAAAKIXEMmE
    %https://docs.google.com/document/d/1OIt0d5Ve4bGTJas2ZIwHXHp7bJlf-1sTJojdwwCfF1I/edit?disco=AAAAG1_7rbk
    
    %\item Requiring students to source tools at home
    %https://docs.google.com/document/d/1OIt0d5Ve4bGTJas2ZIwHXHp7bJlf-1sTJojdwwCfF1I/edit?disco=AAAAG1_7rbc
    
%\end{itemize}

%Experience with access over the quarter.
%\begin{itemize}
%\item Students purchased their own machines, and offered to make them available to other students. This did not materialize. \np{contrast with TAs making lots of things e.g. in RAW}
%https://docs.google.com/document/d/1svv9sfaZ8NtMqLYOEsXdhRuiJxVOhKP2_ZdHqkM_DYM/edit?disco=AAAAKLx4U7w
    
%\item Similar results for Esposito who offered to fabricate parts for students with his machines. Only minority of students with CAD/FAB expertise took advantage of this. Were not able to get their physical parts.
%Paul
    
%\item Option to order parts from campus shop and pick them up was only feasible if you remained in the area.
%https://docs.google.com/document/d/1pi8dNLhy76DvkQUTEmOegwmyoTJq7epPQACGot_1bm8/edit?disco=AAAAG3pc_R4

%\item Ordering from on-demand services takes a long time, and can be delayed. Reduces iteration opportunities, sometimes parts don't arrive.
%https://docs.google.com/spreadsheets/d/1Gp0rCxjDpsg8qkZbCT3GBPLVROr9slUIcWHlF9cNC8Y/edit?disco=AAAAKIXEMlw
%berkeley
%https://docs.google.com/document/d/1EysxU4c-bFz1sgeEMxlNtHQM9mYWu1eXF8402NgCakI/edit?disco=AAAAG4eYUDw

%\item Concern about turning TAs into a fabrication service. ``They signed up to become teaching assistants and that's what they want to do''.
%https://docs.google.com/document/d/1OIt0d5Ve4bGTJas2ZIwHXHp7bJlf-1sTJojdwwCfF1I/edit?disco=AAAAG1wS0lc


%\item Consideration of giving students 3D printer kits due to potential learning opportunities of assembly, tuning, calibration.
%https://docs.google.com/document/d/1OIt0d5Ve4bGTJas2ZIwHXHp7bJlf-1sTJojdwwCfF1I/edit?disco=AAAAKIXEMc4
%\end{itemize}

%The experience of at home fabrication.
%\begin{itemize}
%\item Students who received machines, were able to use them at greater rates, and irregular hours.~\jj{possibly also connect to learning opportunities?}
%https://docs.google.com/document/d/1svv9sfaZ8NtMqLYOEsXdhRuiJxVOhKP2_ZdHqkM_DYM/edit?disco=AAAAKLx5Nvw
%https://docs.google.com/document/d/1svv9sfaZ8NtMqLYOEsXdhRuiJxVOhKP2_ZdHqkM_DYM/edit?disco=AAAAKLx5NvA
%https://docs.google.com/document/d/1bFfPoLLz9gunDBTSW4dAXXWyQPQ3uSr-pSXxcVWAhEs/edit?disco=AAAAG367t44

%\item presence of machines in home could be disruptive to home life for instructors and students.
%https://docs.google.com/document/d/1dJM5lyaog2zqkmpr-qCYtxUG2W1mm2wX1pICl1HFrXw/edit?disco=AAAAG3680Ck

%\item Not ideal to do physical prototyping at home
%https://docs.google.com/document/d/1EysxU4c-bFz1sgeEMxlNtHQM9mYWu1eXF8402NgCakI/edit?disco=AAAAG4KwTo8

%\item Hobbyist craft machines (vinyl cutters) were overly constrained for university level courses. 
%https://docs.google.com/document/d/1bFfPoLLz9gunDBTSW4dAXXWyQPQ3uSr-pSXxcVWAhEs/edit?disco=AAAAG3327NU

%\end{itemize}




%students' accomodation of living space for equipment (1)
%shipping materials & tools (x)
%buying materials & tools (x)
%turning makerspace into jobshop (x)
%logistics (x)
%relying on fabrication services was not very successful/useful... (Ben; Lauren 29-30-31)
%...but sometimes it was (Jessica)

==> sections/findings_sections/fabaccess2.tex <==
Despite minimal planning time, constrained resources, and limited precedent, instructors in the majority of the courses we surveyed worked to create some form of remote digital fabrication access. They were motivated to do so, largely by the unique learning opportunities of hands on fabrication, which we discuss in greater detail in sections \ref{tacit} and \ref{learning}. Instructors were also motivated to meet students' original expectations about engaging in fabrication, in some fashion, however limited. %As \vivek stated why they decided to keep physical making in the second half of \desinv following the shutdown in contrast to other classes that removed physical making:
%\begin{quote}
    %We made a conscious decision \dots hold a certain level of, you know, expectation and outcomes that we wanted to push for\dots
    %\textit{We really wanted to do our best to preserve some of the original intent because we saw there was a lot of desire from students to meet that.}
%\end{quote}

Retaining access to fabrication in the remote setting introduced new forms of labor and management both instructors and students. In several courses instructors~\jj{mark,ben,shelby. more?} required students to source their own tools and materials or re-envision forms of production with at-home materials.  %\markC described the required kit \me: \begin{quote}\textit{We mandated that every student in the class should have a very low tech kit\dots an Exacto knife, hot note, glue guns, some cardboard, masking tape, a ruler.}\end{quote}
Some students were hesitant take on this task during the pandemic, despite the emphasis on supplies that were relatively cheap and widely available. For example, \skylar said he didn't feel inclined “to go to a hardware store and get all of this stuff and leave during quarantine”. %Nevertheless, Shelby saw this limited sourcing context as a creative opportunity to have students re-envisioning forms of production or outcomes with at-home materials.
Precedent for sourcing materials varied across different kinds of departments. The expectation for \me undergrads to assemble their own kits was a new requirement imposed by the shutdown, however, students in art departments were expected to source and pay for their own materials pre-pandemic. \ben- who taught within an art department described these expectation for his students:
\begin{quote}\textit{
We're very upfront\dots projects cost money, you need stuff to make stuff. And and you can work cheap, but you know you need to work with something\dots I'm constantly giving material\dots but it's not like I can supply a whole class.}\end{quote} 
Because of this established expectation, it wasn't a major change for art students in \itp to source materials during the shutdown. Furthermore \ben already had compiled lists of online and local material sources that could aid students in this process.~\jj{could cut this part and quote if it doesn't add much} 

In another form of labor, instructors and students took on the role of digital fabrication technicians. In \raw, one student and two TAs acted as vinyl cutter operators for the other 5 participants. In \itp several students took initiative to create their own job shop. As \ben described:
\begin{quote}
\textit{One person bought an Othermill or a Bantam mill and someone bought 3D printer. [The students] were all sort of like, ``I've got this. If you need a part, I'll run one.''} 
\end{quote}
In \desinv, \paulE fabricated student designs with home 3D printers, in an effort to enable students to ``get in a little bit deeper with some of the projects''.  The model of students and teachers as jobshops~\jj{right word?} created new complications. \markC raised the concern of relying on TAs as technicians rather than educators.
\begin{quote}
    \textit{I need to be a little careful\dots TAs didn't sign up to become a service. They signed up to become teaching assistants and that's what they want to do.}
\end{quote}

Delivering parts to their original designers was non-trivial. \james described how \raw fabricators were not able to mail the parts in time and resorted to photographing the pieces, assembling them and sending the photos to the students. \paulE planed to leave parts at his University for pickup upon the campus reopening, which did not happen. These delivery issues were similar to the challenges instructors encountered when using professional online fabrication services. \me and \desinv used online fabrication vendors, and in both cases students experienced delays in receiving the parts. The logistics of using online vendors disrupted students' ability to personally test and revise their parts. \markC described how \me TAs tested on-demand printed parts for students in the lab \Adam in \desinv explained how shipping delays constrained  students to "only one iteration on the timeline".


A second strategy that took place in one the the surveyed course was to use university maker spaces as a job shops for students to order parts. Students in the \textit{Arch 438X} course were able to order 3D printed or laser cut parts from the CCL at Iowa State University. One student pointed out though that this option was only available for pick up directly at the school which made it “really only an option for like a few people”, adding that “a lot of people that I know moved home, which could be, you know, a couple hours away, um, a couple of States away”. According to this student, it was not clear “how many people actually ended up utilizing that” service. 

Only a few students used this service. According to \ben, the students with machines made  ``one or two things'' for other students but other students chose to ``embrace'' the constraints of limited machine access. Once again only a few students chose to use this service; only 2 of the 21 students had their parts printed by \paulE and users were those most motivated to develop their existing CAD and digital fabrication skills.

%how did they change their curriculum with loss of maker spaces?
In addition to new requirements for sourcing and technical labor, shifting to remote fabrication access required instructors to fundamentally reshaped their curriculum. %The short time frame and limited precedent for remote fabrication led 3 instructors to dramatically alter their curriculum and assignments so they could function without digital fabrication access, while retaining  elements of hands on making or digital fabrication. 
\me's was shifted to focus on collaborative CAD and instructors walked students through basic steps required for digital fabrication or provided remote demonstrations to substitute for hands on access to machines.%:``if you were about to print this, you'd walk over to the printer, you'd stick in your USB''~\jj{can we cut this quote?. it's not so compelling and the point is made without it.. 
~\paulE created an entirely new course (\desma) because his department determined it was infeasible to to teach the original digital fabrication course in a remote format with limited preparation time. Creating a new course gave \paulE freedom to experiment with remote versions of fabrication that including shipping sewing kits, and printing student designs via his home 3D printers as well as hands on forms of making he had not included in in-person classes, like knot tying.

Shifts from access to physical equipment shaped students motivation and ability to pursue course projects that previously required a fabrication component. \lauren in \arch talked about how she was less enthusiastic an assignment for creating stable pen holder for a KUKA robotic arm once she could no longer test it on the actual robot. She described how see the value or the use of developing artifacts that could not be applied to physical equipment. \skylar in \me described being unable to prototype effectively in his home: \begin{quote}
    \textit{I'm not gonna cut a piece of cardboard on my mom's wood dining table\dots There's not really a lot of places in my house where I can do that kind of work.}
\end{quote}



A third investigated strategy was to send hobbyist machines to students. In the case of the R.A.W., the vinyl cutter sent to three people aimed to approximate elements of industry-grade machines. Discussing the relevance of using the vinyl cutter for students interested in space frames, James said that they “were going to basically use paper as a stand in for sheet metal because it was sort of a strength to weight ratio is pretty similar and even formability is quite similar between paper and sheet metal.”

Mark who didn't end up sending 3D printers to his students viewed the 3D printer “kit itself has opportunities for learning about how you assemble things so that the tolerances are actually achieved and alignment and well, lots of issues it can bring up and heating and heat transfer”.

The at-home fabrication strategy showed evidences that students who received machines were able to use them at greater rates, and at irregular hours. Indeed, Ben believed that living with the machine had learning opportunities: 

\begin{quote}
    “The thing I loved about the vinyl cutters more than anything that actually came out of it is that students got to live with the machines. And I think that's really the only way to, to, to get good at it. Right? Like you get a crazy idea and then you immediately make it. And you're like, no, you stay up till four in the morning and you keep working on it. I mean, you somehow learn it inside and out. It starts having quirks that, you know, and that's something that never happened in the past because no one had the machines, they did it here and then they left and there were 10 people behind them waiting for their turn. So access, they had an, you know, parallel access to their machines. And that was huge. I think it just may not have been the machine they wanted, but having total access to something and the time to you know, being trapped in doors with nothing but your vinyl cutter, you know, that learned it.”
\end{quote}

However, the presence of machines at home could also be disruptive to home life for instructors and students. Shelby mentioned zoom calls getting noisy because of the 3D printers running near her, which she could still hear at night when going to bed.

\sbt{living situation here??}

James also mentioned that hobbyist machines, specifically the vinyl cutter, could be overly constraining for university level courses and workshops. Mentioning the automatic scaling done by the machine on larger files, James suggested that the machine "was making a lot of assumptions about us as users, and that were extremely annoying because it wasn't an open software." So, with the participants, they ended up "figuring out the smoothest workflow through and nesting to this size of sheet, even though we could cut it actually cut larger."

A fourth employed strategies involved shipping tools, materials and digitally fabricated parts but the ordering and shipping were often done on the fly with little time for planning ahead. Mark shipped “a marble to everybody” for one assignment and, for another CAD exercise, the instruction team “took all the students' designs, collected them, sent them out to an online 3d fabrication center, 3d hubs, and, uh, and then sent the parts out to the students”. Mark also mailed some testing kits, including a dial gauge and clamps, to each TA "so that they live with their little group could do the test on each crank" designed by their respective students.

%"That was the best we could do in other words, for their six to eight students. So we did send out a, a, a test kit, a dial gauge and, uh, and clamps and so on for each of the TAs, so that they live with their little group could do the test on each crank, but there was just no way we could do, but to each student, we just, we just didn't have time for this last spring." \sbt{add this somehow}



%Paul also sent sewing kits to students who didn't have some already. \sbt{add stuff}




\sbt{need some continuity with previous points} Maker spaces normally provide access to, both, the machines and the expert support for students to learn digital fabrication. Mark mentioned that, for the in-person format of ME102, students “[could] just wander in” the student shops, where “one of the TA’s [would] be holding open shop hours.” ~\jj{not relevant here? learning pathway?}


Most of the surveyed courses were originally designed~\jj{which ones weren't? Can we say a number? e.g. 5 of 6?} around digital fabrication resources in a makerspace. In the rapid onset of the pandemic, instructors had to devise alternative means of access; these alternatives impacted students' motivation, home environment, and ~\jj{summarize}.



==> sections/findings_sections/ourcourses.tex <==
~\jj{title tbd}
\subsubsection{HCDE 598 - Digital Fabrication}
\textit{HCDE 598 - Digital Fabrication} was developed by Nadya within the Human-Centered Design and Engineering Department at the University of Washington. Twenty students enrolled in this quarter-long course in Spring 2020, supported by two TAs. The course introduced students to CAD and prototyping tools for making physical artifacts. For remote instruction students were asked to purchase a \$250 3D printer alongside hand tools (e.g., calipers and Exacto knives) and materials (e.g., 3D printing filament, silicone, plaster, and cardboard.) The total cost per student was around \$350. HCDE 598 was taught via synchronous weekly four hour lectures. To teach students about critical stages in the fabrication pipeline, Nadya developed new assignments that focused on tolerance/fit, compliant mechanisms, system integration, and tooling geometries to forms that were possible with additive fabrication and at-home equipment.


\subsubsection{MAT 594X - Computational Fabrication}~\jj{change to past tense}

MAT 594X was developed by Jennifer as a course in the Media Arts and Technology Graduate Department at the University of California, Santa Barbara. The course included 12 students from media arts and technology and CS. The course emphasized computational fabrication; students used programming languages to design for and control digital fabrication machines. For the Spring 2020 quarter, Jennifer’s own research funds and MAT departmental resources funded low-cost 3D printers and PLA filaments and additional supplies, such as specialty filament, casting materials, and electronic and lighting components, to send to students.The total cost per student ranged between 250 to 350\$. MAT courses included bi-weekly one-hour session held synchronously over Zoom. Weekly course topics and assignments focused on a blend of computational design methods and digital fabrication concepts. However, Jennifer also created new assignments that focused on integrating computer programming with the FDM 3D printing, like requiring students to write programs to procedurally generate G-Code.

\subsection{Analysis of Author Course Outcomes}~\jj{revisit title}
Preliminary analysis of the combined outcomes HCDE 598 and MAT595X suggests that remote instruction with distributed hobbyist 3D printers is a viable method for graduate-level digital fabrication courses. The model reproduced elements of previous makerspace-based courses, particularly with regards to learning to design for machine and material constraints. The model also offered opportunities that were less feasible in shared makerspaces like maintenance and increased iteration. Shifting the workshop to the home environment led to complex forms of personal fabrication, while creating a mix of positive and negative lifestyle changes.  

\subsubsection{Preserving Learning Opportunities of Industrial Equipment with Hobbyist Machines}~\jj{revisit title}
The printers we used lacked many of the features of industrial equipment in university workshops including soluble support material, temperature-controlled build chambers, automated calibration settings. They also had significantly smaller print volumes, slower print speeds, and reduced accuracy. These factors restricted the size, form, and geometry of prints. In the first weeks, students in MAT59X expressed frustration with these limitations and experienced print failures. Several students asked the instructor if more advanced machines would ensure a higher success rate. As the class progressed however, we observed specific ways these machines enabled students to learn how to develop design strategies for specific manufacturing processes. For example, Samuelle Bourgault, an author on this paper, and a student in MAT 594X, printed multiple variations of a design first as a solid part that required an elaborate support structure, and later as a series of modular pieces which required manual assembly, but reduced print time by removing the need for support material. Solen Kiralti created three iterations of a complex print with a procedurally-generated shell and incrementally adjusted the density of the support material until she achieved a successful print with a clean surface finish. Mert Toka, another student in the class researched alternative methods of support structures and slicers. This information was shared and applied by other students throughout the course. ~\jj{nadya- examples from HCDE 598?} Students in both classes experimented with different materials documented and shared machine and slicer settings for different filament types with their peers through slack and discord. 

All digital fabrication machines, regardless of sophistication impose constraints on what can be fabricated. Producing successful products requires learning how to design for these constraints in CAD, how to engage in incremental testing when working with new equipment and materials, and how to systematically adjust machine and CAM parameters to optimize for different geometries. The hobbyist printers imposed more severe constraints than machines we had used in prior courses. Despite these constraints, we observed students adjusting approaches in CAD based on initial machine prints, researching and adjusting machine and material settings, and learning to modify CAM settings based on model geometry. These outcomes suggest similar learning opportunities in integrating CAD, CAM, and machine operation remained present despite our use of hobbyist machines. It is important to also note that students were limited to learning these concepts for one form of additive fabrication. In a makerspace they would have the opportunity to learn CAD-CAM-CNC design processes for different subtractive fabrication processes as well.  This limitation was highlighted in a subtractive CNC CAM assignment in MAT59X where several students ran into errors of scale-- attempting to fabricate parts that were much too large or too small for the target (simulated machine) or similarly, selecting tooling that was much too small. Direct exposure to subtractive milling hardware or machine tooling would have likely provided a way to inform this process in a way that is less feasible through simulation. 

\subsubsection{New Opportunities of At-home 3D printers}
The use of at-home printers also had advantages when compared with how students access machines in a workshop. Unlike staff-managed workshop equipment, individual printers required students to learn about machine maintenance. The Ender 3 Pro requires assembly, and fine-tuning can greatly improve printing outcomes. Nadya built this opportunity directly into her curriculum by making the printer’s assembly and initial calibration one of the first assignments in HCDE 598.  To tune the printers, students relied on instructors' assembly documentation, discussed tips and tricks on Slack, and referred to YouTube videos that demonstrated printer-specific tuning methods. By the end of the spring quarter, students in both courses had tuned and modified their machines to a degree that went significantly beyond the manufacturer documentation. Several students in HCDE 598 exchanged components (such as the fans or power supplies), or 3D printed components to improve performance (such as clips for wire management, holders for work surface illumination, or filament guides). One student in MAT 594X modified the interaction of the printer by creating programs that could stream snippets of print commands in real-time in response to user input via a stylus. These forms of engagement enabled students to familiarize themselves with the machine's implementation details and performance possibilities in a form that would not have been feasible in a shared-use setting.

The at-home setup also allowed for constant access to the printers, which in-turn translated to greater printing output than we had observed with maker-space based classes. Repeated design iterations were common in both courses and went beyond simple optimizations. Victor Allen, a student in HCDE 598, made piles of different design iterations for a camera mount, experimenting with the material strength and incorporating off-the-shelf parts. Weidi Zhang in MAT 594X went through multiple iterations to find a successful printing strategy for sculptures generated from complex photogrammetry data that she had previously only used for digital designs. The resulting prints were accepted into the 2020 IEEE VIS art program. Students were also able to create different kinds of artifacts by developing custom fabrication processes for their machines. In some cases this involved close integration of manual manipulation and machine fabrication. Yanrong Chen in HCDE 598 created a complex sculpture of interlocking chains and birdhouses, which were printed as interlocking structures by pausing the printer at key moments and inserting previously-completed parts. Completing the sculpture involved many tens of hours of print time that were interspersed with regular adjustments or actions made by Yanrong.

Overall, we observed that students achieved higher quality 3D printed parts and greater numbers of design iterations than students in previous classes and workshops who printed on shared machines of comparable quality in shared makerspaces. These observations suggest that constant access to a personal machine directly contributed to the high volume of successful products students created in both classes. Moreover, they provided unique learning opportunities for through maintenance, modification and design iteration. Such opportunities are often obstructed, or altogether hidden in scenarios where machines are shared and maintained by others. 

\subsubsection{Personal Fabrication through Remote Digital Fabrication}
MAT 594X and HCDE 598 provide a new lens to examine approaches to personal fabrication. In addition to facilitating hands-on making in a remote instruction context, shipping printers to students' homes created a situation where students were simultaneously living with printers and creating objects for personal use with them. Both Nadya and Jennifer created assignments that focused on designing objects for the home- including cookie cutters, storage containers and lamps. Several students also took personal intiative to use the printers to design other home goods, or repair or augment existing objects in their home. For example, Mengjia Zhu, a MAT 549X student, created a program that generated designs for a self-watering planter that could be adjusted based on the size of the plant and the desired water immersion level, while incorporating an arbitrary existing outer geometry for the planter basket, and Della Sigrest, in HCDE 598, created a modular lamp that integrated with internal lighting components to create different patterns of light diffusion. 

Projects like Della’s Lamp and Mengjia’s planter conform with many aspects of personal fabrication; these objects were custom-designed and fabricated by the user as opposed to mass-manufactured and purchased. It's important to point out however, that at-home access to the machines did not simplify or accelerate production, or lead to fundamentally new design and manufacturing workflows. To the contrary, such products required students to engage in design workflows that reflect elements of real-world design, manufacturing, and craft. Mengjia used four different CAD software tools, along with custom code tools to produce her finished planter model, and she performed rigorous material testing and machine tuning to ensure that her final design would be water-tight. Della’s final lamp was the result of 12 successive prototypes. At each stage she systematically explored variations of wall thicknesses and geometric patterning. These processes are at odds with product-focused visions of personal fabrication where consumers create custom objects with minimal effort and knowledge. Instead, they show how personal digital fabrication in MAT 594X and HCDE 598 was dependent on deep engagement in learning, design, testing, iteration, and peer support.

\subsubsection{Consequences of Cohabitating with a 3D printer}
In addition to enabling design and production, the presence of the printers in students’ homes also resulted in changes to student’s routines and daily activities. Because students often lived with roommates or occupied small studio apartments, they often kept their printers in their bedrooms. This, coupled with long print times and the fact that the printers generated heat, smells, and machine noises while active, resulted in students coordinating their schedules around their printers. One student described keeping her printer in her bedroom, and was concerned about letting the printer run while she was sleeping. This created a situation where she only had about 10 hours to print each day, which led to additional stress when prints failed or produced undesirable results. Such experiences were not uncommon. Another student had to re-solder the wires on the stepper motors after her cat chewed through them. Another reported that his roommates also had to adjust to the printer and they commented on its constant noise. Our students managed to accommodate the requirements of the printer, but it’s not difficult to envision future scenarios where such constraints would be infeasible and potentially hazardous.

There were elements of at-home 3D printing that provided important forms of stress relief and pleasure. Students in both courses repeatedly expressed their delight at being able to make physical objects and seeing the products made by their classmates. They also talked about the enjoyment and satisfaction they experienced with 3D printing in contrast to the challenges of the quarantine and shutdown, or their experience in other classes. Students remained enthusiastic about the act of physical production in their final project reflections, and many continued to use their printers over the summer. We suspect that the novelty of the at-home 3D printer setup played some role in the students’ excitement. Yet, it’s also possible that at-home fabrication offered relatively rare opportunities for physical interaction when students were otherwise restricted to video conferences, chat, and screen-based work in their classes and research. 


==> sections/findings_sections/ourcourses2.tex <==
Preliminary analysis of the combined outcomes from the author-led courses, \hcde and \mat, suggests that remote instruction with distributed hobbyist 3D printers is a viable method for graduate-level digital fabrication courses. Shifting the workshop to the home led to complex forms of personal fabrication, while creating a mix of positive and negative lifestyle changes. 
 This model offered learning opportunities that were less feasible in shared makerspaces like maintenance and increased iteration. 
 It also enabled the understanding of tacit knowledge associated with the constraints of the 3D printers.

\subsection{Course Summaries}
\nadya and \jennifer's remote fabrication courses used the same remote digital fabrication model of at-home hobbyist 3D printers (at-home machines). Below, we summarize their defining features.

\subsubsection{\hcde~- Digital Fabrication}
\hcde was developed by \nadya in 
%the Human-Centered Design and Engineering Department at the University of Washington. 
an interdisciplinary design and engineering department at a large public school.
Twenty students enrolled in this quarter-long course in Spring 2020, supported by two TAs. The course introduced students to CAD and prototyping tools for making physical artifacts. For remote instruction students were asked to purchase a \$250 3D printer alongside hand tools (e.g., calipers and Exacto knives) and materials (e.g., 3D printing filament, silicone, plaster, and cardboard.) The total cost per student was {$\pm$}\$350. 
%\hcde was taught via synchronous weekly four hour lectures. To teach students about critical stages in the fabrication pipeline, \nadya developed new assignments that focused on tolerance/fit, compliant mechanisms, system integration, and tooling geometries to forms that were possible with additive fabrication and at-home equipment.


\subsubsection{\mat~- Computational Fabrication}
\mat was developed by \jennifer as a course in 
%the Media Arts and Technology Graduate Department at the University of California, Santa Barbara. 
an interdisciplinary art and technology department at a large public school.
The course included 12 students from this department
%media arts and technology 
and from CS. The course emphasized computational fabrication; students used programming languages to design for and control digital fabrication machines. For the Spring 2020 quarter, \jennifer’s own research funds and departmental resources funded low-cost 3D printers and PLA filaments and additional supplies, such as specialty filament, casting materials, and electronic and lighting components, to send to students. The total cost per student ranged from \$250-350. 
%\mat included bi-weekly one-hour session held synchronously over Zoom. Weekly course topics and assignments focused on a blend of computational design methods and digital fabrication concepts. However, \jennifer also created new assignments that focused on integrating computer programming with the FDM 3D printing, like requiring students to write programs to procedurally generate G-Code.

%The model reproduced elements of previous makerspace-based courses, particularly with regards to learning to design for machine and material constraints. The model also offered opportunities that were less feasible in shared makerspaces like maintenance and increased iteration. Shifting the workshop to the home environment led to complex forms of personal fabrication, while creating a mix of positive and negative lifestyle changes.


\subsection{Impacts of At-Home 3D Printers}
%~\jj{check tense}

% - All cohabitation section goes in that
% - Personal fabrication
%    - Student could built effective first home stuff for them
Shipping printers to students' homes created a situation where students were simultaneously living with printers and creating objects for personal use with them. Several students also took personal initiative or assignment contexts to use the printers to design home goods or to repair or augment existing objects in their home. One \mat student created a program that generated designs for a customizable self-watering planter, and one student in \hcde created a modular lamp integrated with internal lighting components to create different patterns of light diffusion. 

Projects such as these conform with many aspects of personal fabrication; these objects were custom-designed and fabricated by their maker as opposed to mass-manufactured and purchased. It is important to point out, however, that at-home access to the machines did not simplify or accelerate production, or lead to fundamentally new design and manufacturing workflows. To the contrary, such products required students to engage in design workflows that reflect elements of real-world design, manufacturing, and craft. Both projects involved deep engagement in learning, design, testing, iteration, and peer support. These processes are at odds with product-focused visions of personal fabrication where consumers create custom objects with minimal effort and knowledge. 

The presence of the printers in students’ homes also resulted in changes to student’s routines and daily activities. Because students often lived with roommates or occupied small studio apartments, they often kept their printers in their bedrooms. This, coupled with long print times and the fact that the printers generated heat, smells, and machine noises while active, resulted in students coordinating their schedules around their printers and additional stress when prints failed. One student reported that his roommates also had to adjust to the printer and they commented on its constant noise. Another student had to re-solder the wires on the stepper motors after her cat chewed through them. Our students managed to accommodate the requirements of the printer, but it is not difficult to envision future scenarios where such constraints would be infeasible and potentially hazardous. There were also elements of at-home 3D printing that provided important forms of stress relief and pleasure. Students in both courses repeatedly expressed their delight at being able to make physical objects and seeing the products made by their classmates. We suspect that the novelty of the at-home 3D printer setup played some role in the students’ excitement. Yet, it is also possible that at-home fabrication offered relatively rare opportunities for physical interaction when students were otherwise restricted to video conferences, chat, and screen-based work in their classes and research.

\subsection{Learning Opportunities of Hobbyist 3D Printers}
%~\jj{check tense}
The use of at-home printers also had unique opportunities when compared with how students access machines in a workshop. Unlike staff-managed workshop equipment, individual printers required students to learn about machine maintenance. Though the Ender 3 Pro printer required assembly, fine-tuning it can greatly improve printing outcomes. \nadya built this opportunity directly into her curriculum by making the printer’s assembly and initial calibration one of the first assignments in \hcde. By the end of the spring quarter, students in both courses had tuned and modified their machines to a degree that went significantly beyond the manufacturer documentation. Several students in \hcde upgraded components (such as the fans or power supplies) or 3D printed components to improve performance (such as clips for wire management, holders for work surface illumination, or filament guides). These forms of engagement enabled students to familiarize themselves with the machine's implementation details and performance possibilities in a form that would not have been feasible in a shared-use setting.
%One student in \mat modified the interaction of the printer by creating programs that could stream snippets of print commands in real-time in response to user input via a stylus.

The at-home setup also allowed for constant access to the printers, which in turn translated to the possibility for students to iterate extensively on their designs. Repeated design iterations were common in both courses and went beyond simple optimizations. One student in \mat went through multiple iterations to find a successful printing strategy for sculptures generated from complex photogrammetry data that she had previously only used for digital designs. The resulting prints were accepted into a top-tier visualization conference. Students were also able to create different kinds of artifacts by developing custom fabrication processes for their machines. In some cases this involved close integration of manual manipulation and machine fabrication. One student created a complex sculpture of interlocking chains and birdhouses, which were printed as interlocking structures by pausing the printer at key moments and inserting previously-completed parts (shown in Figure \ref{fig:figure1}A). Completing the sculpture involved many tens of hours of print time that were interspersed with regular adjustments or actions made by the student.
%One student in \hcde made piles of different design iterations for a camera mount, experimenting with the material strength and incorporating off-the-shelf parts. 

%As the class progressed however, we observed specific ways these machines enabled students to learn how to develop design strategies for specific manufacturing processes. For example, Samuelle Bourgault, an author on this paper, and a student in MAT 594X, printed multiple variations of a design first as a solid part that required an elaborate support structure, and later as a series of modular pieces which required manual assembly, but reduced print time by removing the need for support material. Solen Kiralti created three iterations of a complex print with a procedurally-generated shell and incrementally adjusted the density of the support material until she achieved a successful print with a clean surface finish. Mert Toka, another student in the class researched alternative methods of support structures and slicers. This information was shared and applied by other students throughout the course. ~\jj{nadya- examples from HCDE 598?}

Overall, at-home 3D printers provided unique learning opportunities for maintenance, modification and design iteration. Such opportunities are often obstructed when machines are shared and maintained by others.

\subsection{Gaining Tacit Knowledge Remotely}
%~\sbt{working title}
%~\jj{check tense}
The use of at-home 3D printers enabled students to work across CAD, CAM, and CNC throughout the courses. We observed students iterating in CAD based on initial machine prints, learning to modify CAM settings based on model geometry, and iterating on machine and material settings based on settings they looked up and tuned. 
%\sbt{Not sure to understand this following sentence syntactically!!} \np{updated}
These outcomes suggest similar learning opportunities in integrating CAD, CAM, and machine operation remained present despite our use of hobbyist machines. It is important to also note that students were limited to learning these concepts with one form of additive fabrication. In a makerspace they would have the opportunity to learn CAD-CAM-CNC design processes for additional subtractive fabrication processes.  This limitation was highlighted in a subtractive CNC/CAM assignment in \mat where several students ran into errors of scale---attempting to fabricate parts that were much too large or too small for the target (simulated machine) or similarly, selecting tooling that was much too small. Direct exposure to subtractive milling hardware or machine tooling would have likely provided a way to inform this process in a way that is less feasible through simulation. 

All digital fabrication machines, regardless of sophistication, place constraints on what can be fabricated. Producing successful products requires learning how to design for these constraints in CAD, how to engage in incremental testing when working with new equipment and materials, and how to systematically adjust machine and CAM parameters to optimize for different geometries. The hobbyist printers imposed more severe constraints than machines we had used in prior courses but still enabled students to develop these forms of knowledge.



==> sections/internalfindings.tex <==
\input{sections/findings_sections/ourcourses2}

